Compact Extra Dimensions in Quantum Mechanics

Extra-dimensions are a common topic in popular descriptions of theoretical physics with which undergraduate student most often have no contact in physics courses. This paper shows how students could be introduced to this topic by presenting an approach to two basic consequences of the presence of compact extra-dimensions based on undergraduate-level physics. The insensibility of low-energy physics to compact extra dimensions is illustrated in the context of non-relativistic quantum mechanics and the prediction of Kaluza-Klein excitations of particles is discussed in the framework of relativistic wave-equations. An exercise that could be used as a follow-up to the "particle in a box" is proposed.

==> content/lapl.tex <==
In this appendix, we provide a short explanation of why the momentum-squared operator on a curved manifold is given by the Laplacian operator, whose general definition we will also provide.

\subsection{Geometry}
The geometry of a curved space is entirely contained in a 2D matrix, called the metric and often designated as $g$, which encodes how distances are measured in the space.
Let us consider a system of coordinates in our space $(\zeta_1,\dots,\zeta_n)$, and specify a point $Z$ at coordinates $(\zeta_1^0,\dots,\zeta_n^0)$.
If we consider an infinitesimally close point $Z'$, at coordinates $(\zeta_1^0+\text{d}\zeta_1,\dots,\zeta_n^0\text{d}\zeta_n)$, the distance separating these two points is given by the $g$-induced bilinear product:

\begin{equation}
\text{dist}(Z,Z') = \sum_{i,j} \text{d}\zeta_i\times \text{d}\zeta_j\times g_{ij}.
\end{equation}

Essentially, the metric gives us a way to translate vectors to norms, which is what we want when we consider the squared momentum.
In curved spaces, the metric will depend on position, while a property of flat spaces is that there exists a choice of coordinate system that makes the metric a position-independent identity matrix.

The metric also helps us define the general Laplacian operator, in a parametrization independent way:

\begin{equation}
  \Delta = \sum \left(g^{-1}\right)_{ij} \partial_i \partial_j,
\end{equation}

When changing coordinates $\zeta_i\to x_j$, the metric transforms as $g_{ij}=\partial$
which yields the usual expression $\partial_x^2+\partial_y^2+\partial_z^2$ in flat 3D space.
The metric on the sphere is

\begin{equation}
  \begin{pmatrix}
    R^2 & 0 \\
    0 & R^2 \sin^2 \theta
  \end{pmatrix}
\end{equation}

and again we find the expression in Eq.\ref{s2lapl}: $$\frac{1}{R^2} \partial_\theta^2 + \frac{1}{R^2\sin^2}\partial_\phi^2.$$

\subsection{Momentum in curved spaces}

The interpretation of the derivative as the quantum-mechanical momentum operator is conserved in curved spaces at least locally.
Locally, one can always approximate a space as flat, that is to say, around a point $M$, there is always a choice of coordinates $\left\{\xi_k\right\}$ such that $M$ is at $(0,\cdots,0)$ and the metric takes a nearly flat form $g_{ij}(\left\{ \xi_k \right\}) = \delta_{ij} +  {\cal O}(\xi_k)$.
Around point $M$ at least, we can define operators for

